Grounding Driving VLA via Inverse Kinematics

Counterfactual obstacle insertion exposes blind planning in representative Driving VLAs: their trajectories remain largely unchanged despite a vehicle appearing directly ahead. An empirically calibrated bias-variance analysis identifies how ego-predictable training examples admit a shortcut through ego status and commands. We address this failure with an inverse-kinematics-inspired architecture that anchors trajectory decoding on current and predicted future visual states. First, a next visual state prediction objective that requires the LLM to predict the future visual scene provides dense visual supervision and suppresses shortcut paths. Second, a separate Inverse Kinematics Network (a cross-attention-based conditional diffusion model) that takes only the current and future visual states as input is designed to suppress reliance on ego status and textual shortcuts during trajectory decoding. Our 0.5B model achieves state-of-the-art trajectory planning performance on NAVSIM-v1, NAVSIM-v2, and nuScenes using cameras alone, without LiDAR or a BEV encoder. Against the matched OpenDriveVLA* baseline, it improves NAVSIM PDMS and EPDMS by 19.0 and 20.4 points, respectively. Controlled ablations and intervention analyses support improved use of visual features, with future-state prediction sharpening hazard-specific responses.

==> tables/ego_status_split.tex <==
\begin{table}[t]
\centering
\caption{
\textbf{Stratified evaluation on nuScenes \emph{val} ($n=6019$) by ego-status difficulty}, following the criterion of Li \etal\cite{li2024ego}.
For each sample, we measure the GT-relative ADE of an ego-status-only constant-velocity + constant-yaw-rate extrapolation (\emph{ego-status gap}); the top $30\%$ ($\geq 2.14$\,m, $n=1{,}805$) forms the \emph{VisionCritical} subset and the bottom $30\%$ ($\leq 0.668$\,m, $n=1{,}805$) forms the \emph{EgoDominated} subset.
We compare three models: the original OpenDriveVLA \cite{zhou2025opendrivevla} (\textit{DriveVLA-orig}), a text-only variant trained with the visual stream architecturally removed (\textit{TextOnly-novis}), and our model (\textit{Ours}).
We report UniAD avg.\ L2 (m) and Collision (\%); \textbf{bold} = best per column.
}
\label{tab:ego_status_split}
\setlength{\tabcolsep}{4pt}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{DriveVLA-orig} & \multicolumn{2}{c}{TextOnly-novis} & \multicolumn{2}{c}{Ours} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
Subset & L2$\downarrow$ & Coll.$\downarrow$ & L2$\downarrow$ & Coll.$\downarrow$ & L2$\downarrow$ & Coll.$\downarrow$ \\
\midrule
Full ($n{=}6{,}019$)              & 0.347 & 0.090 & 0.308 & 0.078 & \textbf{0.063} & \textbf{0.044} \\
EgoDominated ($n{=}1{,}805$)      & 0.166 & 0.012 & 0.190 & \textbf{0.003} & \textbf{0.049} & 0.060 \\
VisionCritical ($n{=}1{,}805$)    & 0.429 & 0.172 & 0.371 & 0.078 & \textbf{0.066} & \textbf{0.011} \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

